High-Speed Accurate Robot Control using Learned Forward Kinodynamics and Non-linear Least Squares Optimization

Accurate control of robots at high speeds requires a control system that can take into account the kinodynamic interactions of the robot with the environment. Prior works on learning inverse kinodynamic (IKD) models of robots have shown success in capturing the complex kinodynamic effects. However, the types of control problems these approaches can be applied to are limited only to that of following pre-computed kinodynamically feasible trajectories. In this paper we present Optim-FKD, a new formulation for accurate, high-speed robot control that makes use of a learned forward kinodynamic (FKD) model and non-linear least squares optimization. Optim-FKD can be used for accurate, high speed control on any control task specifiable by a non-linear least squares objective. Optim-FKD can solve for control objectives such as path following and time-optimal control in real time, without needing access to pre-computed kinodynamically feasible trajectories. We empirically demonstrate these abilities of our approach through experiments on a scale one-tenth autonomous car. Our results show that Optim-FKD can follow desired trajectories more accurately and can find better solutions to optimal control problems than baseline approaches.

==> math_formulation_reference.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Mathematical Formulation Reference}
This section is not intended to go in the paper. It just lists the full mathematical formulation in its entirety. When writing the technical section, take chunks from here and follow along with surrounding text.

Probabilistic forward kinodynamic response, and learned approximations $f_\theta, \Sigma_\phi$ thereof:
\begin{align}
p(x_{t+1}|x_t, u_t) &= \mathcal{N}(f(x_t, u_t), \Sigma(x_t, u_t))\\
 &\simeq \mathcal{N}(f_\theta(x_t, u_t), \Sigma_\theta(x_t, u_t))
\end{align}
Likelihood over a trajectory rollout with finite horizon $T$:
\begin{align}
p(x_{1:T}|x_0, u_{1:T}) &= \prod_{t=0}^{T-1}p(x_{t+1}|x_t, u_t)\\
&= \prod_{t=0}^{T-1}\mathcal{N}(f(x_t, u_t), \Sigma(x_t, u_t))\\
&\simeq \prod_{t=0}^{T-1}\mathcal{N}(f_\theta(x_t, u_t), \Sigma_\phi(x_t, u_t))
\end{align}
Optimization objective, given a desired path $\bar{x}_{1:T}$:
\begin{align}
u_{1:T}^* = \argmax_{u_{1:T}} E_{p(x_{1:T}|x_0, u_{1:T})}\left[J(x_{1:T},\bar{x}_{1:T},u_{1:T}) \right]
\end{align}
where $E_{p(x)}[C(x)]$ is the expected value of $C(x)$ under the distribution $p(x)$.
Possible variants of the optimization objective $J$ include the path-following objective
\begin{align}
J(x_{1:T},\bar{x}_{1:T},u_{1:T}) = ||x_{1:T}, \bar{x}_{1:T}||_{H}
\end{align}
where $||\cdot, \cdot||_{H}$ is the Hausdorff distance.
Another variant is the timed path-following objective, where the robot is desired to be at specific locations at specific points of time,
\begin{align}
J(x_{1:T},\bar{x}_{1:T},u_{1:T}) = \sum_{i=1}^{T} ||x_i - \bar{x}_i||^2.
\end{align}
A receding horizon objective that desires the robot to end at the desired trajectory with a weak trajectory-following regularization is,
\begin{align}
J(x_{1:T},\bar{x}_{1:T},u_{1:T}) = ||x_T-\bar{x}_T||^2 + \eta  ||x_{1:T-1}, \bar{x}_{1:T-1}||_{H},
\end{align}
where $\eta$ is a hyper-parameter that trades off following the desired trajectory accurately for reaching the final state on the trajectory.

Under a special case of the optimization objective $J$, solving for the optimal control reduces to a non-linear least squares problem.
Let $J$ be decomposed as
\begin{align}
J(x_{1:T},\bar{x}_{1:T},u_{1:T}) = \sum_{i=1}^{T} J_i(||x_i - \bar{x}_i||^2),
\end{align}
where every $J_i\forall i\in [1,T]$ is a monotonic positive semidefinite function.
Under this simplification, the optimal control is given by,

